SCENE: Self-Labeled Counterfactuals for Extrapolating to Negative Examples

Detecting negatives (such as non-entailment relationships, unanswerable questions, and false claims) is an important and challenging aspect of many natural language understanding tasks. Though manually collecting challenging negative examples can help models detect them, it is both costly and domain-specific. In this work, we propose Self-labeled Counterfactuals for Extrapolating to Negative Examples (SCENE), an automatic method for synthesizing training data that greatly improves models' ability to detect challenging negative examples. In contrast with standard data augmentation, which synthesizes new examples for existing labels, SCENE can synthesize negative examples zero-shot from only positive ones. Given a positive example, SCENE perturbs it with a mask infilling model, then determines whether the resulting example is negative based on a self-training heuristic. With access to only answerable training examples, SCENE can close 69.6% of the performance gap on SQuAD 2.0, a dataset where half of the evaluation examples are unanswerable, compared to a model trained on SQuAD 2.0. Our method also extends to boolean question answering and recognizing textual entailment, and improves generalization from SQuAD to ACE-whQA, an out-of-domain extractive QA benchmark.

==> Tables/ablation_short.tex <==
\begin{table}[t!]
\small 
\renewcommand{\arraystretch}{0.9}
\setlength\tabcolsep{9.2pt}
%\captionsetup{font=small}
    \centering
    \begin{tabular}{c | g  c | g  c}
    \hline
        \multirow{2}*{Method} & \multicolumn{2}{c|}{SQuAD 2.0} & \multicolumn{2}{c}{ACE-whQA}\tstrut \bstrut \\
        \hhline{~|--|--}
        &  $EM$ & $F_1$ & $EM$ & $F_1$ \tstrut \bstrut\\
        \hline
        Assume NoAns &  68.5 & 70.5 & 60.8 & ~62.6 \tstrut  \\ 
        $\uparrow$ w/o Retr &  65.0 & 67.4 & 58.8 & 60.1 \\
        Only NoAns &  67.9 & 70.7 & 67.4 & 70.6 \\
        No Filter &  67.5  & 69.9 & 65.9 & 68.1\\
        \underline{\emph{SCENE} (ours)} & \textbf{68.9}  & \textbf{71.8}  & \textbf{69.8} & \textbf{73.1} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study} on different filtering and labeling strategies. The full SCENE pipeline achieves the best performance both in-domain and out-of-domain. }
    \label{tab:ablation-short}
\end{table}

==> Tables/ace_whqa.tex <==
\begin{table*}[t]
\small 
\setlength\tabcolsep{4pt}
%\captionsetup{font=small}
    \centering
    \begin{tabular}{c |  c | g  c | g  c | g  c}
        \toprule
        \multirow{ 3}*{Training Set} & \multirow{ 3}*{Method} & \multicolumn{2}{c|}{Has Answer} & \multicolumn{2}{c|}{No Answer} & \multicolumn{2}{c}{Average} \tstrut \bstrut \\
        \hhline{~|~|--|--|--|}
        & & $EM$ & $F_1$ & \makecell{{\small Competitive} \\$EM$/$F_1$} & \makecell{{\small Non-Competitive} \\$EM$/$F_1$} & $EM$ & $F_1$ \tstrut \bstrut\\
        \hline 
        \multirow{6}*{\makecell{SQuAD 1.1 
        %\\ \cite{rajpurkar-etal-2016-squad}
        }} & RoBERTa\textsubscript{\tiny Base} & 79.13 (0.52) & 86.80 (0.82) & 1.07 (1.24) & 7.86 (7.78) & 41.80 (2.10) & ~45.63 (1.85) \tstrut \\
        & RoBERTa\textsubscript{\tiny Base} (best threshold) & 62.89 (3.45) & 68.15 (3.54) & 72.16 (3.80) & 95.39 (1.34) & 73.33 (1.24) & 75.96 (1.19) \\
        & Shuffle & 56.02 (7.72) & 63.99 (7.47) & 71.22 (7.73) & 90.51 (3.52) & 68.44 (1.11) & 72.43 (0.96) \\
        %\cline{2-8} 
        & Shuf + Pert & 58.96 (3.67) & 65.08 (4.86) & 69.75 (5.01) & 87.26 (2.66) & 68.73 (0.18) & 71.79 (0.55)\\
        %\cline{2-8} 
        & Retrieval & 53.78 (5.95) & 60.28 (6.46) & 76.97 (6.34) & 95.66 (1.94) & 70.05 (0.91) & 73.30 (1.16) \\
        & Retr +  Pert & 62.61 (3.27) & 69.86 (3.59) & 70.15 (4.10) & 94.31 (1.15) & \textbf{72.42 (0.60)} & ~\textbf{76.05 (0.51)} \bstrut \\
        \hline 
        \multirow{4}*{\makecell{SQuAD 2.0 
        %\\ \cite{rajpurkar-etal-2018-know}
        }} & RoBERTa\textsubscript{\tiny Base}  & 49.86 (2.92) & 56.61 (3.84) & 80.05 (3.66) & 92.55 (1.50) & 68.08 (0.25) & ~71.46 (0.69) \tstrut \\
        %\cline{2-8} 
        & Perturbation & 48.04 (1.39) & 55.39 (0.98) & 78.45 (1.37) & 92.01 (1.01) & 66.63 (0.65) & 70.31 (0.43) \\
        & Retrieval & 55.60 (1.39) & 61.48 (1.62) & 73.09 (0.87) & 92.95 (0.69) & 69.31 (0.84) & 72.25 (0.95) \\
        %\cline{2-8} 
        & Retr +  Pert & 51.40 (3.44) & 59.06 (4.33) & 72.82 (4.15) & 90.65 (2.32) & 66.57 (0.38) & 70.40 (0.80) \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Evaluation on ACE-whQA} with the best threshold for non-answerable probabilities (except the RoBERTa\textsubscript{Base} on SQuAD 1.1 where the model never saw non-answerable questions). {\color{red} [ADD MORE TEXT]}}
    \label{tab:whqa}
\end{table*}

==> Tables/squad_v2_two_deci.tex <==
\begin{table*}[t]
\small 
%\captionsetup{font=small}
\setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{c |  c | g  c | g  c | g  c}
        \toprule
        \multirow{ 2}*{Training Set} & \multirow{ 2}*{Method} & \multicolumn{2}{c|}{Has Answer} & \multicolumn{2}{c|}{No Answer} & \multicolumn{2}{c}{Average} \tstrut \bstrut \\
        \hhline{~|~|--|--|--|}
        & & $EM$ & $F_1$ & $EM$ & $F_1$ & $EM$ & $F_1$ \tstrut \bstrut\\
        \hline 
        \multirow{5}*{\makecell{SQuAD 1.1 %\\ \cite{rajpurkar-etal-2016-squad}
        }} & No Augmentation & 84.40 (0.22) & 91.51 (0.12) & 0.00 (0.00) & 0.00 (0.00) & 42.14 (0.11) & ~45.69 (0.06) \tstrut \bstrut \\
        %\hhline{~-|--|--|--|}
        & Shuffle & 84.08 (0.28) & 91.32 (0.14) & 3.37 (0.28) & 3.37 (0.28) & 43.66 (0.08) & 47.28 (0.08)\\ 
        & Shuf + SCENE & 80.08 (0.21) & 86.54 (0.09) & 40.84 (1.65) & 40.84 (1.65) & 60.43 (0.81) & 63.66 (0.79)\\
        %\hhline{~-|--|--|--|}
        & Retrieval  & 79.34 (0.08) & 85.45 (0.23) & 43.08 (0.73) & 43.08 (0.73) & 61.18 (0.38) & 64.24 (0.35)\\ 
        & Retr + SCENE & 75.75 (0.55) & 81.36 (0.56) & 62.18 (0.87) & 62.18 (0.87) & 68.95 (0.17) & ~71.75 (0.16)   
        %\\ & Perm + Retr + Pert & 75.43 (0.27) & 80.94 (0.24) & 64.27 (0.75) & 64.27 (0.75) & 69.84 (0.36) & 72.59 (0.32) 
        \bstrut\\
        \hline 
        \multirow{2}*{\makecell{SQuAD 2.0 %\\ \cite{rajpurkar-etal-2018-know}
        }} & No Augmentation & 78.19 (0.22) & 84.58 (0.34) & 81.82 (0.54) & 81.82 (0.54) & 80.01 (0.16) & ~83.20 (0.10) \tstrut \\
        %\hhline{~-|--|--|--|}
        & SCENE & 76.25 (0.25) & 82.19 (0.19) & 84.59 (0.40) & 84.59 (0.40) & 80.42 (0.08) & 83.39 (0.11)\\ 
        %\hhline{~-|--|--|--|}
        % & Retrieval  & 74.43 (0.17) & 80.44 (0.06) & 86.55 (0.13) & 86.55 (0.13) & 80.50 (0.05) & 83.50 (0.04) \\ 
        % & Retr + Pert & 72.51 (0.34) & 77.84 (0.42) & 88.02 (0.32) & 88.02 (0.32) & 80.28 (0.10) & 82.94 (0.11)\\
        % & Retr + Pert {\tiny  ($\lambda = 0.5$)} & 74.56 (0.32) & 80.27 (0.40) & 87.02 (0.13) & 87.02 (0.13) & 80.80 (0.13) & 83.65 (0.17) \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Evaluation on SQuAD 2.0}. Training on positive-only SQuAD 1.1, SCENE with Retrieval can close 69.5\% of the gap compared with an oracle model trained on SQuAD 2.0. We report the mean and standard deviation (in parentheses) over 3 runs.}
    \label{tab:squad}
\end{table*}
